Trinary Tools for Continuously Valued Binary Classifiers

Classification methods for binary (yes/no) tasks often produce a continuously valued score. Machine learning practitioners must perform model selection, calibration, discretization, performance assessment, tuning, and fairness assessment. Such tasks involve examining classifier results, typically using summary statistics and manual examination of details. In this paper, we provide an interactive visualization approach to support such continuously-valued classifier examination tasks. Our approach addresses the three phases of these tasks: calibration, operating point selection, and examination. We enhance standard views and introduce task-specific views so that they can be integrated into a multi-view coordination (MVC) system. We build on an existing comparison-based approach, extending it to continuous classifiers by treating the continuous values as trinary (positive, unsure, negative) even if the classifier will not ultimately use the 3-way classification. We provide use cases that demonstrate how our approach enables machine learning practitioners to accomplish key tasks.

==> 1-intro.tex <==
\ifieee\IEEEPARstart{A}{ssessment}\else Assessment \fi
\xspace of classifier performance is important. It plays a role in model selection (i.e., choosing the most appropriate classifier and tuning it appropriately) but also in assessing whether a classifier is good enough (Can it be trusted?) or fair (Does it treat subgroups equivalently?). Assessment is also a valuable tool in developing classifiers, providing insights on errors that can help tune and debug models, and check data.
However, assessment is also very situational. Classifiers involve tradeoffs, balancing between different types of errors (false positives, false negatives, and \emph{rejection} where the classifier chooses not to make a decision because of uncertainty), and on different ``locality'' of errors (i.e., having the likelihood of error depend on the item being classified). 

In practice, classifier developers assess performance by looking at how decisions are made over a test population. They must consider not only the costs of errors, but also their likelihood in practice.
Assessment is enhanced by detailed analysis of the classifier results: rather than relying on summary statistics (e.g., precision, recall, F1), practitioners examine the results closely to gain insights, for example by identifying specific items or subgroups that are problematic, patterns in the results that suggest insights on how the model works, or correlations among results. Such detailed analysis is commonly performed manually using scripting with the development workflow. However, a variety of recent interactive visualization approaches have been introduced to help with the detailed assessment of classifier results.



% Working with classifiers involves making tradeoffs: classifiers must be tuned to balance between the different types of errors they may make (false positives, false negatives, and rejection where the classifier chooses not to make a decision because it is too uncertain). Each situation may have different tradeoffs between these error types.

When classifiers compute continuously valued scores, there are further opportunities and challenges in assessment. These scores are often thresholded to provide a binary decision. In some cases, the score is also used for \emph{rejection} \cite{chowOptimumRecognitionError1970,landgrebeInteractionClassificationReject2006} where the classifier chooses not to make a decision. We term such classifiers as \emph{trinary} as they provide one of three results (positive, unsure, negative). Assessing classifier scores involves three phases of tasks: \emph{calibration,} where the scores are examined to assess how well they correspond to possible decisions; \emph{operating point selection,} where the thresholds for decisions and (optionally) rejection are determined; and \emph{assessment} where the decisions made by the classifier are examined.
However, support for these tasks with continuously valued classifiers is limited. Summary statistics of continuous classifiers tend to be complex (e.g., P/R or ROC curves or area-under-curve metrics) and no standards have emerged for considering rejection \cite{condessaPerformanceMeasuresClassification2017}. Users must consider additional parameters (e.g., decision thresholds) and questions (e.g., do the outputs meaningfully quantify desired qualities such as confidence or uncertainty?).

Current methods address specific tasks. While these tools enhance the baseline of scripting within standard workflows, they do not extend to the diverse range of tasks users encounter, either by adapting to new situations or combining effectively to provide detailed analyses. We seek a more comprehensive approach using a combination of task-specific solutions and standard views with coordination mechanisms.

Our target audience is machine learning practioners, ranging from students to experience developers and researchers. This audience is familiar with the standard terminology, metrics, and charts. From a design perspective, this means an approach must include the common views that such users demand for basic tasks, but extend them to integrate into workflows that support tasks that are inconvenient to do with standard script-based tooling. For example, users typically create standard curves (ROC or P/R) to assess a classifier's correctness and estimate good threshold values, but they may need augmentations to these standard views to help focus on relevant examples and new views that can help them evaluate rejection criteria.

In this paper, we describe an approach to support tasks involving the assessment of continuously valued binary classifiers. Our key idea is that by integrating support for trinary (yes/unsure/no) decision making, we can support specific tasks for rejection classifiers, but also use this trinary classification as a strategy to organize analysis where the ultimate classifier will not use rejection.
Our approach integrates the three phases of analysis: calibration, operating point selection and detailed analysis. By providing coordinated tools for these phases, they can be combined, for example using detailed analysis at varied operating points to understand the ramifications of calibration.
Because these tools are used to estimate hyper-parameters (thresholds), the approach integrates sampling to allow separate sets for estimation and validation.

We focus on the common case of continuous valued \emph{binary} classifiers. Similarly, we focus on the classifier results: we treat the classifiers as black boxes and consider only input/output pairs. Our approach considers making detailed comparisons, \emph{between} different classifiers as well as \emph{within} a classifier (i.e., comparing different groups of items). Our work targets machine learning practitioners who need to assess classifiers based on their results. However, some of our methods may be useful in aiding other stakeholders who may need to tune thresholds to adapt classifier tradeoffs to their specific needs or appreciate the specific ramifications of a classifier's performance.

Our core contribution is an approach to assessment of continuously-valued binary classifiers that is sufficiently flexible to adapt to a wide range of tasks, yet allows for detail oriented analysis.
We introduce the strategy of using trinary classification to provide a  system that addresses score interpretation tasks, including specific views and coordination mechanisms.
We make a number of specific contributions.
First, we provide a set of views for assessing the calibration and operating point tradeoffs in classifiers. These views include extensions of standard views that enhance their ability to coordinate in workflows, as well as novel views that provide improved presentation of the interaction between parameters.
Second, we extend existing work on detailed classifier assessment to better handle the situations that arise. This includes views that allow for group-based assessment of multi-valued binary classifiers, mechanisms that enhance aggregate analysis views for more detailed analysis, and better handling of skewed test distributions.
Third, we show how new sampling features can be added to assessment tools in order to help users avoid over fitting their analyses.
Our approach, including these novel techniques, has been integrated into the \sysname classifier comparison and analysis system, which provides an open source prototype of the ideas.

